The Kinetic Sunyaev-Zel'dovich Effect from Reionization: Simulated Full Sky Maps at Arcminute Resolution

The kinetic Sunyaev-Zel'dovich (kSZ) effect results from Thomson scattering by coherent flows in the reionized intergalactic medium. We present new results based on ray-tracing a 10 Gpc scale simulation at 2-3 Mpc scale resolution to create a full sky kSZ map. The simulation includes, self-consistently, the effects of reionization on scales corresponding to multipoles $10\lesssim\ell\lesssim{5000}$. We separate the kSZ map into Doppler ($\mathbf{v}$), Ostriker-Vishniac ($\delta\mathbf{v}$), patchy ($x\mathbf{v}$), and third-order ($x\delta\mathbf{v}$) components, and compute explicitly all the auto and cross correlations (e.g., $\langle\mathbf{v}\mathbf{v}\rangle$, $\langle\delta\mathbf{v}{x}\mathbf{v}\rangle$, etc.) that contribute to the total power. We find a complex dependence on the duration of reionization at $\ell\sim{300}$ and evidence for a non-negligible (10-30 per cent) contribution from connected four point ionization-velocity correlations, $\langle{x}\mathbf{v}x\mathbf{v}\rangle_c$, that are usually neglected in analytical models. We also investigate the Doppler-large scale structure (LSS) correlation, focusing on two different probes: (1) cross power spectra with linearly biased tracers of LSS and (2) cold spots from infall onto large, rare \ion{H}{2} regions centered on peaks in the matter distribution at redshifts $z>10$. Finally, the reionization history can be reconstructed at 5-10$\sigma$ significance by correlating 21-cm maps with existing CMB temperature maps at $\ell\!<\!500$ --sophisticated velocity reconstruction methods can probe the distribution of electrons in the IGM by using combined CMB and LSS measurements well into the epoch of reionization. The resulting kSZ maps have been made publicly available at http://www.cita.utoronto.ca/~malvarez/research/ksz-data.

==> bib.tex <==
\begin{thebibliography}{55}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\expandafter\ifx\csname href\endcsname\relax
  \def\href#1#2{}\fi
\expandafter\ifx\csname urllinklabel\endcsname\relax
  \def\urllinklabel{[LINK]}\fi
\expandafter\ifx\csname adsurllinklabel\endcsname\relax
  \def\adsurllinklabel{[ADS]}\fi

\bibitem[{{Adshead} \& {Furlanetto}(2008)}]{2008MNRAS.384..291A}
{Adshead}, P.~J. \& {Furlanetto}, S.~R. 2008, \mnras, 384, 291


\bibitem[{{Aghanim} {et~al.}(2008){Aghanim}, {Majumdar}, \&
  {Silk}}]{2008RPPh...71f6902A}
{Aghanim}, N., {Majumdar}, S., \& {Silk}, J. 2008, Reports on Progress in
  Physics, 71, 066902


\bibitem[{{Alvarez} \& {Abel}(2012)}]{2012ApJ...747..126A}
{Alvarez}, M.~A. \& {Abel}, T. 2012, \apj, 747, 126


\bibitem[{{Alvarez} {et~al.}(2006){Alvarez}, {Komatsu}, {Dor{\'e}}, \&
  {Shapiro}}]{2006ApJ...647..840A}
{Alvarez}, M.~A., {Komatsu}, E., {Dor{\'e}}, O., \& {Shapiro}, P.~R. 2006,
  \apj, 647, 840


\bibitem[{{Battaglia} {et~al.}(2013){Battaglia}, {Natarajan}, {Trac}, {Cen}, \&
  {Loeb}}]{2013ApJ...776...83B}
{Battaglia}, N., {Natarajan}, A., {Trac}, H., {Cen}, R., \& {Loeb}, A. 2013,
  \apj, 776, 83


\bibitem[{{Calabrese} {et~al.}(2014){Calabrese}, {Hlo{\v z}ek}, {Battaglia},
  {Bond}, \& et~al.}]{2014JCAP...08..010C}
{Calabrese}, E., {Hlo{\v z}ek}, R., {Battaglia}, N., {Bond}, J.~R., \& et~al.
  2014, \jcap, 8, 10


\bibitem[{{Chibisov} \& {Ozernoy}(1969)}]{1969ApL.....3..189C}
{Chibisov}, G.~V. \& {Ozernoy}, L.~M. 1969, \aplett, 3, 189


\bibitem[{{Chluba} and {Sunyaev}(2004)}]{2004A\&{A}...424..389C}
{Chluba}, J. and {Sunyaev}, R.~A. 2004, \aap, 424, 389


\bibitem[{{Cooray}(2004)}]{2004PhRvD..70f3509C}
{Cooray}, A. 2004, \prd, 70, 063509


\bibitem[{{Dodelson} \& {Jubas}(1995)}]{1995ApJ...439..503D}
{Dodelson}, S. \& {Jubas}, J.~M. 1995, \apj, 439, 503


\bibitem[{{Furlanetto} {et~al.}(2006){Furlanetto}, {Oh}, \&
  {Briggs}}]{2006PhR...433..181F}
{Furlanetto}, S.~R., {Oh}, S.~P., \& {Briggs}, F.~H. 2006, \physrep, 433, 181


\bibitem[{{George} {et~al.}(2015){George}, {Reichardt}, \&
  et~al.}]{2015ApJ...799..177G}
{George}, E.~M., {Reichardt}, C.~L., \& et~al. 2015, \apj, 799, 177


\bibitem[{{Giannantonio} \& {Crittenden}(2007)}]{2007MNRAS.381..819G}
{Giannantonio}, T. \& {Crittenden}, R. 2007, \mnras, 381, 819


\bibitem[{{Gnedin} \& {Jaffe}(2001)}]{2001ApJ...551....3G}
{Gnedin}, N.~Y. \& {Jaffe}, A.~H. 2001, \apj, 551, 3


\bibitem[{{Gruzinov} \& {Hu}(1998)}]{1998ApJ...508..435G}
{Gruzinov}, A. \& {Hu}, W. 1998, \apj, 508, 435


\bibitem[{{Hill} {et~al.}(2015){Hill}, {Battaglia}, {Chluba}, {Ferraro},
  {Schaan}, \& {Spergel}}]{2015arXiv150701583H}
{Hill}, J.~C., {Battaglia}, N., {Chluba}, J., {Ferraro}, S., {Schaan}, E., \&
  {Spergel}, D.~N. 2015, ArXiv e-prints


\bibitem[{{Hinshaw} {et~al.}(2013){Hinshaw}, {Larson}, {Komatsu}, \& {Spergel,
  D.~N., et al.}}]{2013ApJS..208...19H}
{Hinshaw}, G., {Larson}, D., {Komatsu}, E., \& {Spergel, D.~N., et al.} 2013,
  \apjs, 208, 19


\bibitem[{{Hu}(2000)}]{2000ApJ...529...12H}
{Hu}, W. 2000, \apj, 529, 12


\bibitem[{{Hu} \& {Dodelson}(2002)}]{2002ARA\&{A}..40..171H}
{Hu}, W. \& {Dodelson}, S. 2002, \araa, 40, 171


\bibitem[{{Hu} {et~al.}(1994){Hu}, {Scott}, \& {Silk}}]{1994PhRvD..49..648H}
{Hu}, W., {Scott}, D., \& {Silk}, J. 1994, \prd, 49, 648


\bibitem[{{Iliev} {et~al.}(2007){Iliev}, {Pen}, {Bond}, {Mellema}, \&
  {Shapiro}}]{2007ApJ...660..933I}
{Iliev}, I.~T., {Pen}, U.-L., {Bond}, J.~R., {Mellema}, G., \& {Shapiro}, P.~R.
  2007, \apj, 660, 933


\bibitem[{{Jaffe} \& {Kamionkowski}(1998)}]{1998PhRvD..58d3001J}
{Jaffe}, A.~H. \& {Kamionkowski}, M. 1998, \prd, 58, 043001


\bibitem[{{Jeli{\'c}} {et~al.}(2010){Jeli{\'c}}, {Zaroubi}, {Aghanim},
  {Douspis}, {Koopmans}, {Langer}, {Mellema}, {Tashiro}, \&
  {Thomas}}]{2010MNRAS.402.2279J}
{Jeli{\'c}}, V., {Zaroubi}, S., {Aghanim}, N., {Douspis}, M., {Koopmans},
  L.~V.~E., {Langer}, M., {Mellema}, G., {Tashiro}, H., \& {Thomas}, R.~M.
  2010, \mnras, 402, 2279


\bibitem[{{Kaiser}(1984)}]{1984ApJ...282..374K}
{Kaiser}, N. 1984, \apj, 282, 374


\bibitem[{{Kaiser}(1987)}]{1987MNRAS.227....1K}
---. 1987, \mnras, 227, 1


\bibitem[{{Knox} {et~al.}(1998){Knox}, {Scoccimarro}, \&
  {Dodelson}}]{1998PhRvL..81.2004K}
{Knox}, L., {Scoccimarro}, R., \& {Dodelson}, S. 1998, Physical Review Letters,
  81, 2004


\bibitem[{{Ma} \& {Fry}(2002)}]{2002PhRvL..88u1301M}
{Ma}, C.-P. \& {Fry}, J.~N. 2002, Physical Review Letters, 88, 211301


\bibitem[{{McQuinn} {et~al.}(2005){McQuinn}, {Furlanetto}, {Hernquist}, {Zahn},
  \& {Zaldarriaga}}]{2005ApJ...630..643M}
{McQuinn}, M., {Furlanetto}, S.~R., {Hernquist}, L., {Zahn}, O., \&
  {Zaldarriaga}, M. 2005, \apj, 630, 643


\bibitem[{{Mesinger} {et~al.}(2012){Mesinger}, {McQuinn}, \&
  {Spergel}}]{2012MNRAS.422.1403M}
{Mesinger}, A., {McQuinn}, M., \& {Spergel}, D.~N. 2012, \mnras, 422, 1403


\bibitem[{{Ostriker} \& {Vishniac}(1986)}]{1986ApJ...306L..51O}
{Ostriker}, J.~P. \& {Vishniac}, E.~T. 1986, \apjl, 306, L51


\bibitem[{{Park} {et~al.}(2015){Park}, {Komatsu}, {Shapiro}, {Koda}, \&
  {Mao}}]{2015arXiv150605177P}
{Park}, H., {Komatsu}, E., {Shapiro}, P.~R., {Koda}, J., \& {Mao}, Y. 2015,
  ArXiv e-prints


\bibitem[{{Park} {et~al.}(2013){Park}, {Shapiro}, {Komatsu}, {Iliev}, {Ahn}, \&
  {Mellema}}]{2013ApJ...769...93P}
{Park}, H., {Shapiro}, P.~R., {Komatsu}, E., {Iliev}, I.~T., {Ahn}, K., \&
  {Mellema}, G. 2013, \apj, 769, 93


\bibitem[{{Peiris} \& {Spergel}(2000)}]{2000ApJ...540..605P}
{Peiris}, H.~V. \& {Spergel}, D.~N. 2000, \apj, 540, 605


\bibitem[{{Pen} {et~al.}(2012){Pen}, {Sheth}, {Harnois-Deraps}, {Chen}, \&
  {Li}}]{2012arXiv1202.5804P}
{Pen}, U.-L., {Sheth}, R., {Harnois-Deraps}, J., {Chen}, X., \& {Li}, Z. 2012,
  ArXiv e-prints


\bibitem[{{Planck Collaboration et al}(2015)}]{2015arXiv150201589P}
{Planck Collaboration et al}. 2015, arXiv:1502.01589


\bibitem[{{Reichardt} {et~al.}(2012){Reichardt}, {Shaw}, \&
  et~al.}]{2012ApJ...755...70R}
{Reichardt}, C.~L., {Shaw}, L., Z.~O., \& et~al. 2012, \apj, 755, 70


\bibitem[{{Salvaterra} {et~al.}(2005){Salvaterra}, {Ciardi}, {Ferrara}, \&
  {Baccigalupi}}]{2005MNRAS.360.1063S}
{Salvaterra}, R., {Ciardi}, B., {Ferrara}, A., \& {Baccigalupi}, C. 2005,
  \mnras, 360, 1063


\bibitem[{{Santos} {et~al.}(2003){Santos}, {Cooray}, {Haiman}, {Knox}, \&
  {Ma}}]{2003ApJ...598..756S}
{Santos}, M.~G., {Cooray}, A., {Haiman}, Z., {Knox}, L., \& {Ma}, C.-P. 2003,
  \apj, 598, 756


\bibitem[{{Sunyaev}(1977)}]{1977SvAL....3..268S}
{Sunyaev}, R.~A. 1977, Soviet Astronomy Letters, 3, 268


\bibitem[{{Sunyaev}(1978)}]{1978IAUS...79..393S}
{Sunyaev}, R.~A. in , IAU Symposium, Vol.~79, Large Scale Structures in the
  Universe, ed. M.~S. {Longair}J.~{Einasto}, 393--402


\bibitem[{{Sunyaev} \& {Zeldovich}(1970{\natexlab{a}})}]{1970Ap\&SS...7....3S}
{Sunyaev}, R.~A. \& {Zeldovich}, Y.~B. 1970{\natexlab{a}}, \apss, 7, 3


\bibitem[{{Sunyaev} \& {Zeldovich}(1970{\natexlab{b}})}]{1970CoASP...2...66S}
---. 1970{\natexlab{b}}, Comments on Astrophysics and Space Physics, 2, 66


\bibitem[{{Sunyaev} \& {Zeldovich}(1972)}]{1972CoASP...4..173S}
---. 1972, Comments on Astrophysics and Space Physics, 4, 173


\bibitem[{{Tashiro} {et~al.}(2010){Tashiro}, {Aghanim}, {Langer}, {Douspis},
  {Zaroubi}, \& {Jelic}}]{2010MNRAS.402.2617T}
{Tashiro}, H., {Aghanim}, N., {Langer}, M., {Douspis}, M., {Zaroubi}, S., \&
  {Jelic}, V. 2010, \mnras, 402, 2617


\bibitem[{{Tashiro} {et~al.}(2011){Tashiro}, {Aghanim}, {Langer}, {Douspis},
  {Zaroubi}, \& {Jeli{\'c}}}]{2011MNRAS.414.3424T}
{Tashiro}, H., {Aghanim}, N., {Langer}, M., {Douspis}, M., {Zaroubi}, S., \&
  {Jeli{\'c}}, V. 2011, \mnras, 414, 3424


\bibitem[{{Trac} {et~al.}(2011){Trac}, {Bode}, \&
  {Ostriker}}]{2011ApJ...727...94T}
{Trac}, H., {Bode}, P., \& {Ostriker}, J.~P. 2011, \apj, 727, 94


\bibitem[{{Valageas} {et~al.}(2001){Valageas}, {Balbi}, \&
  {Silk}}]{2001A\&{A}...367....1V}
{Valageas}, P., {Balbi}, A., \& {Silk}, J. 2001, \aap, 367, 1


\bibitem[{{Visbal} \& {Loeb}(2012)}]{2012JCAP...05..007V}
{Visbal}, E. \& {Loeb}, A. 2012, \jcap, 5, 7


\bibitem[{{Vishniac}(1987)}]{1987ApJ...322..597V}
{Vishniac}, E.~T. 1987, \apj, 322, 597


\bibitem[{{Weymann}(1966)}]{1966ApJ...145..560W}
{Weymann}, R. 1966, \apj, 145, 560


\bibitem[{{Zahn} {et~al.}(2012){Zahn}, {Reichardt}, {Shaw}, \& {Lidz, A., et
  al.}}]{2012ApJ...756...65Z}
{Zahn}, O., {Reichardt}, C.~L., {Shaw}, L., \& {Lidz, A., et al.} 2012, \apj,
  756, 65


\bibitem[{{Zahn} {et~al.}(2005){Zahn}, {Zaldarriaga}, {Hernquist}, \&
  {McQuinn}}]{2005ApJ...630..657Z}
{Zahn}, O., {Zaldarriaga}, M., {Hernquist}, L., \& {McQuinn}, M. 2005, \apj,
  630, 657


\bibitem[{{Zel'dovich} {et~al.}(1972){Zel'dovich}, {Illarionov}, \&
  {Syunyaev}}]{1972JETP...35..643Z}
{Zel'dovich}, Y.~B., {Illarionov}, A.~F., \& {Syunyaev}, R.~A. 1972, Soviet
  Journal of Experimental and Theoretical Physics, 35, 643


\bibitem[{{Zeldovich} \& {Sunyaev}(1969)}]{1969Ap\&SS...4..301Z}
{Zeldovich}, Y.~B. \& {Sunyaev}, R.~A. 1969, \apss, 4, 301


\bibitem[{{Zhang} {et~al.}(2004){Zhang}, {Pen}, \&
  {Trac}}]{2004MNRAS.347.1224Z}
{Zhang}, P., {Pen}, U.-L., \& {Trac}, H. 2004, \mnras, 347, 1224


\end{thebibliography}

